Pioneering Precision in Lumbar Spine MRI Segmentation with Advanced Deep Learning and Data Enhancement

This study presents an advanced approach to lumbar spine segmentation using deep learning techniques, focusing on addressing key challenges such as class imbalance and data preprocessing. Magnetic resonance imaging (MRI) scans of patients with low back pain are meticulously preprocessed to accurately represent three critical classes: vertebrae, spinal canal, and intervertebral discs (IVDs). By rectifying class inconsistencies in the data preprocessing stage, the fidelity of the training data is ensured. The modified U-Net model incorporates innovative architectural enhancements, including an upsample block with leaky Rectified Linear Units (ReLU) and Glorot uniform initializer, to mitigate common issues such as the dying ReLU problem and improve stability during training. Introducing a custom combined loss function effectively tackles class imbalance, significantly improving segmentation accuracy. Evaluation using a comprehensive suite of metrics showcases the superior performance of this approach, outperforming existing methods and advancing the current techniques in lumbar spine segmentation. These findings hold significant advancements for enhanced lumbar spine MRI and segmentation diagnostic accuracy.

==> ref.tex <==
@article{roudsari2010lumbar,
  title={Lumbar spine MRI for low back pain: indications and yield},
  author={Roudsari, Bahman and Jarvik, Jeffrey G},
  journal={American Journal of Roentgenology},
  volume={195},
  number={3},
  pages={550--559},
  year={2010},
  publisher={Am Roentgen Ray Soc}
}

@article{sheehan2010magnetic,
  title={Magnetic resonance imaging for low back pain: indications and limitations},
  author={Sheehan, NJ},
  journal={Postgraduate medical journal},
  volume={86},
  number={1016},
  pages={374--378},
  year={2010},
  publisher={Oxford University Press}
}

@article{katz2006lumbar,
  title={Lumbar disc disorders and low-back pain: socioeconomic factors and consequences},
  author={Katz, Jeffrey N},
  journal={JbJs},
  volume={88},
  number={suppl\_2},
  pages={21--24},
  year={2006},
  publisher={LWW}
}

@article{van2002mri,
  title={MRI of the postoperative lumbar spine},
  author={Van Goethem, J and Parizel, P and Jinkins, J},
  journal={Neuroradiology},
  volume={44},
  pages={723--739},
  year={2002},
  publisher={Springer}
}
@article{patil2013medical,
  title={Medical image segmentation: a review},
  author={Patil, Dinesh D and Deore, Sonal G},
  journal={International Journal of Computer Science and Mobile Computing},
  volume={2},
  number={1},
  pages={22--27},
  year={2013}
}
@article{aggarwal2011role,
  title={Role of segmentation in medical imaging: A comparative study},
  author={Aggarwal, Preeti and Vig, Renu and Bhadoria, Sonali and Dethe, CG},
  journal={International Journal of Computer Applications},
  volume={29},
  number={1},
  pages={54--61},
  year={2011},
  publisher={International Journal of Computer Applications, 244 5 th Avenue,\# 1526, New~…}
}
@article{cheng2021deep,
  title={Deep learning: an update for radiologists},
  author={Cheng, Phillip M and Montagnon, Emmanuel and Yamashita, Rikiya and Pan, Ian and Cadrin-Ch{\^e}nevert, Alexandre and Perdig{\'o}n Romero, Francisco and Chartrand, Gabriel and Kadoury, Samuel and Tang, An},
  journal={Radiographics},
  volume={41},
  number={5},
  pages={1427--1445},
  year={2021},
  publisher={Radiological Society of North America}
}
@article{zhou2021review,
  title={A review of deep learning in medical imaging: Imaging traits, technology trends, case studies with progress highlights, and future promises},
  author={Zhou, S Kevin and Greenspan, Hayit and Davatzikos, Christos and Duncan, James S and Van Ginneken, Bram and Madabhushi, Anant and Prince, Jerry L and Rueckert, Daniel and Summers, Ronald M},
  journal={Proceedings of the IEEE},
  volume={109},
  number={5},
  pages={820--838},
  year={2021},
  publisher={IEEE}
}
@phdthesis{patel2023improving,
  title={Improving Segmentation Pipelines for Medical Imaging using Deep Learning},
  author={Patel, Jay Biren},
  year={2023},
  school={Massachusetts Institute of Technology}
}
@article{najjar2023redefining,
  title={Redefining radiology: a review of artificial intelligence integration in medical imaging},
  author={Najjar, Reabal},
  journal={Diagnostics},
  volume={13},
  number={17},
  pages={2760},
  year={2023},
  publisher={MDPI}
}
@article{11van2024lumbar,
  title={Lumbar spine segmentation in MR images: a dataset and a public benchmark},
  author={van der Graaf, Jasper W and van Hooff, Miranda L and Buckens, Constantinus FM and Rutten, Matthieu and van Susante, Job LC and Kroeze, Robert Jan and de Kleuver, Marinus and van Ginneken, Bram and Lessmann, Nikolas},
  journal={Scientific Data},
  volume={11},
  number={1},
  pages={264},
  year={2024},
  publisher={Nature Publishing Group UK London}
}
@article{12wang2022automatic,
  title={Automatic segmentation of lumbar spine MRI images based on improved attention U-net},
  author={Wang, Shuai and Jiang, Zhengwei and Yang, Hualin and Li, Xiangrong and Yang, Zhicheng},
  journal={Computational Intelligence and Neuroscience},
  volume={2022},
  number={1},
  pages={4259471},
  year={2022},
  publisher={Wiley Online Library}
}
@article{13silvoster2020efficient,
  title={Efficient segmentation of lumbar intervertebral disc from MR images},
  author={Silvoster M, Leena and Mathusoothana S. Kumar, Retnaswami},
  journal={IET Image Processing},
  volume={14},
  number={13},
  pages={3076--3083},
  year={2020},
  publisher={Wiley Online Library}
}

@article{14peng2021convenient,
  title={A convenient and stable vertebrae instance segmentation method for transforaminal endoscopic surgery planning},
  author={Peng, Wuke and Li, Liang and Liang, Libin and Ding, Hui and Zang, Lei and Yuan, Shuo and Wang, Guangzhi},
  journal={International Journal of Computer Assisted Radiology and Surgery},
  volume={16},
  number={8},
  pages={1263--1276},
  year={2021},
  publisher={Springer}
}
@inproceedings{15van2022segmentation,
  title={Segmentation of vertebrae and intervertebral discs in lumbar spine MR images with iterative instance segmentation},
  author={van der Graaf, Jasper W and van Hooff, Miranda L and Buckens, Constantinus FM and Lessmann, Nikolas},
  booktitle={Medical Imaging 2022: Image Processing},
  volume={12032},
  pages={909--913},
  year={2022},
  organization={SPIE}
}
@inproceedings{unetronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={Medical image computing and computer-assisted intervention--MICCAI 2015: 18th international conference, Munich, Germany, October 5-9, 2015, proceedings, part III 18},
  pages={234--241},
  year={2015},
  organization={Springer}
}
@inproceedings{unet++zhou2018unet++,
  title={Unet++: A nested u-net architecture for medical image segmentation},
  author={Zhou, Zongwei and Rahman Siddiquee, Md Mahfuzur and Tajbakhsh, Nima and Liang, Jianming},
  booktitle={Deep Learning in Medical Image Analysis and Multimodal Learning for Clinical Decision Support: 4th International Workshop, DLMIA 2018, and 8th International Workshop, ML-CDS 2018, Held in Conjunction with MICCAI 2018, Granada, Spain, September 20, 2018, Proceedings 4},
  pages={3--11},
  year={2018},
  organization={Springer}
}
@article{attention_unet_oktay2018attention,
  title={Attention u-net: Learning where to look for the pancreas},
  author={Oktay, Ozan and Schlemper, Jo and Folgoc, Loic Le and Lee, Matthew and Heinrich, Mattias and Misawa, Kazunari and Mori, Kensaku and McDonagh, Steven and Hammerla, Nils Y and Kainz, Bernhard and others},
  journal={arXiv preprint arXiv:1804.03999},
  year={2018}
}

@article{datasetvan2023spider,
  title={SPIDER-Lumbar spine segmentation in MR images: a dataset and a public benchmark},
  author={van der Graaf, JW and others},
  journal={Zenodo https://doi. org/10.5281/zenodo},
  volume={10159290},
  year={2023}
}

@article{3D_slicer_fedorov20123d,
  title={3D Slicer as an image computing platform for the Quantitative Imaging Network},
  author={Fedorov, Andriy and Beichel, Reinhard and Kalpathy-Cramer, Jayashree and Finet, Julien and Fillion-Robin, Jean-Christophe and Pujol, Sonia and Bauer, Christian and Jennings, Dominique and Fennessy, Fiona and Sonka, Milan and others},
  journal={Magnetic resonance imaging},
  volume={30},
  number={9},
  pages={1323--1341},
  year={2012},
  publisher={Elsevier}
}

@article{MRI_richardson2005pharmaceutical,
  title={Pharmaceutical applications of magnetic resonance imaging (MRI)},
  author={Richardson, J Craig and Bowtell, Richard W and M{\"a}der, Karsten and Melia, Colin D},
  journal={Advanced drug delivery reviews},
  volume={57},
  number={8},
  pages={1191--1209},
  year={2005},
  publisher={Elsevier}
}

\@article{MRI_Detection_kirkham2006good,
  title={How good is MRI at detecting and characterising cancer within the prostate?},
  author={Kirkham, Alexander PS and Emberton, Mark and Allen, Clare},
  journal={European urology},
  volume={50},
  number={6},
  pages={1163--1175},
  year={2006},
  publisher={Elsevier}
}

@inproceedings{surgical_1_warfield1998real,
  title={Real-time image segmentation for image-guided surgery},
  author={Warfield, Simon K and Jolesz, Ferenc A and Kikinis, Ron},
  booktitle={SC'98: Proceedings of the 1998 ACM/IEEE Conference on Supercomputing},
  pages={42--42},
  year={1998},
  organization={IEEE}
}

@article{Surgical_2_li2021medical,
  title={Medical image segmentation in oral-maxillofacial surgery},
  author={Li, Jianning and Erdt, Marius and Janoos, Firdaus and Chang, Ti-chiun and Egger, Jan},
  journal={Computer-Aided Oral and Maxillofacial Surgery},
  pages={1--27},
  year={2021},
  publisher={Elsevier}
}

@article{identifying_abnormalities_1_yanagisawa2023convolutional,
  title={Convolutional neural network-based skin image segmentation model to improve classification of skin diseases in conventional and non-standardized picture images},
  author={Yanagisawa, Yuta and Shido, Kosuke and Kojima, Kaname and Yamasaki, Kenshi},
  journal={Journal of Dermatological Science},
  volume={109},
  number={1},
  pages={30--36},
  year={2023},
  publisher={Elsevier}
}
@article{identifying_abnormalities_2_narayan2023comprehensive,
  title={A comprehensive review of various approach for medical image segmentation and disease prediction},
  author={Narayan, Vipul and Faiz, Mohammad and Mall, Pawan Kumar and Srivastava, Swapnita},
  journal={Wireless Personal Communications},
  volume={132},
  number={3},
  pages={1819--1848},
  year={2023},
  publisher={Springer}
}

@article{radio_1_wataya2023radiologists,
  title={Radiologists with and without deep learning--based computer-aided diagnosis: comparison of performance and interobserver agreement for characterizing and diagnosing pulmonary nodules/masses},
  author={Wataya, Tomohiro and Yanagawa, Masahiro and Tsubamoto, Mitsuko and Sato, Tomoharu and Nishigaki, Daiki and Kita, Kosuke and Yamagata, Kazuki and Suzuki, Yuki and Hata, Akinori and Kido, Shoji and others},
  journal={European Radiology},
  volume={33},
  number={1},
  pages={348--359},
  year={2023},
  publisher={Springer}
}

@article{radio_2_neves2024shedding,
  title={Shedding light on ai in radiology: A systematic review and taxonomy of eye gaze-driven interpretability in deep learning},
  author={Neves, Jos{\'e} and Hsieh, Chihcheng and Nobre, Isabel Blanco and Sousa, Sandra Costa and Ouyang, Chun and Maciel, Anderson and Duchowski, Andrew and Jorge, Joaquim and Moreira, Catarina},
  journal={European Journal of Radiology},
  pages={111341},
  year={2024},
  publisher={Elsevier}
}

@article{radio_3_liao2023deep,
  title={Deep learning approaches to automatic radiology report generation: A systematic review},
  author={Liao, Yuxiang and Liu, Hantao and Spasi{\'c}, Irena},
  journal={Informatics in Medicine Unlocked},
  volume={39},
  pages={101273},
  year={2023},
  publisher={Elsevier}
}
@article{Class_imbalance_better_model_tholke2023class,
  title={Class imbalance should not throw you off balance: Choosing the right classifiers and performance metrics for brain decoding with imbalanced data},
  author={Th{\"o}lke, Philipp and Mantilla-Ramos, Yorguin-Jose and Abdelhedi, Hamza and Maschke, Charlotte and Dehgan, Arthur and Harel, Yann and Kemtur, Anirudha and Berrada, Loubna Mekki and Sahraoui, Myriam and Young, Tammy and others},
  journal={NeuroImage},
  volume={277},
  pages={120253},
  year={2023},
  publisher={Elsevier}
}

@article{UNET_2_siddique2021u,
  title={U-net and its variants for medical image segmentation: A review of theory and applications},
  author={Siddique, Nahian and Paheding, Sidike and Elkin, Colin P and Devabhaktuni, Vijay},
  journal={IEEE access},
  volume={9},
  pages={82031--82057},
  year={2021},
  publisher={IEEE}
}
@article{glorot_1_chumachenko2022feedforward,
  title={Feedforward neural networks initialization based on discriminant learning},
  author={Chumachenko, Kateryna and Iosifidis, Alexandros and Gabbouj, Moncef},
  journal={Neural Networks},
  volume={146},
  pages={220--229},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{Glorot_2_aguirre2019improving,
  title={Improving weight initialization of relu and output layers},
  author={Aguirre, Diego and Fuentes, Olac},
  booktitle={Artificial Neural Networks and Machine Learning--ICANN 2019: Deep Learning: 28th International Conference on Artificial Neural Networks, Munich, Germany, September 17--19, 2019, Proceedings, Part II 28},
  pages={170--184},
  year={2019},
  organization={Springer}
}

@article{leaky_relu_1_mastromichalakis2020alrelu,
  title={ALReLU: A different approach on Leaky ReLU activation function to improve Neural Networks Performance},
  author={Mastromichalakis, Stamatis},
  journal={arXiv preprint arXiv:2012.07564},
  year={2020}
}

@inproceedings{leaky_relu_2_dubey2019comparative,
  title={Comparative study of convolution neural network’s relu and leaky-relu activation functions},
  author={Dubey, Arun Kumar and Jain, Vanita},
  booktitle={Applications of Computing, Automation and Wireless Systems in Electrical Engineering: Proceedings of MARC 2018},
  pages={873--880},
  year={2019},
  organization={Springer}
}
@inproceedings{dying_relu_1_douglas2018relu,
  title={Why RELU units sometimes die: Analysis of single-unit error backpropagation in neural networks},
  author={Douglas, Scott C and Yu, Jiutian},
  booktitle={2018 52nd Asilomar Conference on Signals, Systems, and Computers},
  pages={864--868},
  year={2018},
  organization={IEEE}
}
@article{classimbalance_1_yeung2022unified,
  title={Unified focal loss: Generalising dice and cross entropy-based losses to handle class imbalanced medical image segmentation},
  author={Yeung, Michael and Sala, Evis and Sch{\"o}nlieb, Carola-Bibiane and Rundo, Leonardo},
  journal={Computerized Medical Imaging and Graphics},
  volume={95},
  pages={102026},
  year={2022},
  publisher={Elsevier}
}
@article{classimbalance_3_cui2024unified,
  title={A Unified Approach Addressing Class Imbalance in Magnetic Resonance Image for Deep Learning Models},
  author={Cui, Lijuan and Li, Dengao and Yang, Xiaofeng and Liu, Chao and Yan, Xiaoting},
  journal={IEEE Access},
  year={2024},
  publisher={IEEE}
}

@article{Metric_various_wang2024revisiting,
  title={Revisiting evaluation metrics for semantic segmentation: Optimization and evaluation of fine-grained intersection over union},
  author={Wang, Zifu and Berman, Maxim and Rannen-Triki, Amal and Torr, Philip and Tuia, Devis and Tuytelaars, Tinne and Gool, Luc V and Yu, Jiaqian and Blaschko, Matthew},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}
@article{metric_dice_liu2024we,
  title={Do we really need dice? The hidden region-size biases of segmentation losses},
  author={Liu, Bingyuan and Dolz, Jose and Galdran, Adrian and Kobbi, Riadh and Ayed, Ismail Ben},
  journal={Medical Image Analysis},
  volume={91},
  pages={103015},
  year={2024},
  publisher={Elsevier}
}
@article{metric_3_opitz2024closer,
  title={A Closer Look at Classification Evaluation Metrics and a Critical Reflection of Common Evaluation Practice},
  author={Opitz, Juri},
  journal={Transactions of the Association for Computational Linguistics},
  volume={12},
  pages={820--836},
  year={2024},
  publisher={MIT Press 255 Main Street, 9th Floor, Cambridge, Massachusetts 02142, USA~…}
}

@article{Batch_Normalization_santurkar2018does,
  title={How does batch normalization help optimization?},
  author={Santurkar, Shibani and Tsipras, Dimitris and Ilyas, Andrew and Madry, Aleksander},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@article{dropout_srivastava2014dropout,
  title={Dropout: a simple way to prevent neural networks from overfitting},
  author={Srivastava, Nitish and Hinton, Geoffrey and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  journal={The journal of machine learning research},
  volume={15},
  number={1},
  pages={1929--1958},
  year={2014},
  publisher={JMLR. org}
}

@article{Leaky_hu2021handling,
  title={Handling vanishing gradient problem using artificial derivative},
  author={Hu, Zheng and Zhang, Jiaojiao and Ge, Yun},
  journal={IEEE Access},
  volume={9},
  pages={22371--22377},
  year={2021},
  publisher={IEEE}
}

@inproceedings{golorot_aguirre2019improving,
  title={Improving weight initialization of relu and output layers},
  author={Aguirre, Diego and Fuentes, Olac},
  booktitle={Artificial Neural Networks and Machine Learning--ICANN 2019: Deep Learning: 28th International Conference on Artificial Neural Networks, Munich, Germany, September 17--19, 2019, Proceedings, Part II 28},
  pages={170--184},
  year={2019},
  organization={Springer}
}

@inproceedings{focal_lin2017focal,
  title={Focal loss for dense object detection},
  author={Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2980--2988},
  year={2017}
}

@inproceedings{dice_zhao2020rethinking,
  title={Rethinking dice loss for medical image segmentation},
  author={Zhao, Rongjian and Qian, Buyue and Zhang, Xianli and Li, Yang and Wei, Rong and Liu, Yang and Pan, Yinggang},
  booktitle={2020 IEEE International Conference on Data Mining (ICDM)},
  pages={851--860},
  year={2020},
  organization={IEEE}
}

@article{spi1_yang2023rau,
  title={RAU-Net: U-Net network based on residual multi-scale fusion and attention skip layer for overall spine segmentation},
  author={Yang, Zhaomin and Wang, Qi and Zeng, Jianchao and Qin, Pinle and Chai, Rui and Sun, Dong},
  journal={Machine Vision and Applications},
  volume={34},
  number={1},
  pages={10},
  year={2023},
  publisher={Springer}
}
@article{spi_2petrakis2024lunar,
  title={Lunar ground segmentation using a modified U-net neural network},
  author={Petrakis, Georgios and Partsinevelos, Panagiotis},
  journal={Machine Vision and Applications},
  volume={35},
  number={3},
  pages={50},
  year={2024},
  publisher={Springer}
}

